MEDCOD: A Medically-Accurate, Emotive, Diverse, and Controllable Dialog System

We present MEDCOD, a Medically-Accurate, Emotive, Diverse, and Controllable Dialog system with a unique approach to the natural language generator module. MEDCOD has been developed and evaluated specifically for the history taking task. It integrates the advantage of a traditional modular approach to incorporate (medical) domain knowledge with modern deep learning techniques to generate flexible, human-like natural language expressions. Two key aspects of MEDCOD's natural language output are described in detail. First, the generated sentences are emotive and empathetic, similar to how a doctor would communicate to the patient. Second, the generated sentence structures and phrasings are varied and diverse while maintaining medical consistency with the desired medical concept (provided by the dialogue manager module of MEDCOD). Experimental results demonstrate the effectiveness of our approach in creating a human-like medical dialogue system. Relevant code is available at https://github.com/curai/curai-research/tree/main/MEDCOD

==> sections/quals.tex <==
\begin{table*}[]
\begin{tabular}{l|l|l}
\hline
 Expert & Ours-No-Emote & Ours \\
  \hline
  \hline
  \multicolumn{3}{l}{Finding: recurrent headache  Emote: affirmative } \\
  \hline
Do you have headaches that come and go often? & Do you have headaches that occur on a regular basis?  & Thanks for the input. Does you  headache keep coming back?\\
& Are your headaches recurring? & Okay. Is your headache recurrent?  \\
\end{tabular}
\label{tab:qual_comparison}
\caption{Qualitative comparison of generated questions by the three NLG models. Note the lack of diversity in the \textbf{Expert} model and lack of emotion in the \textbf{Ours-no-Emote} model. The questions generated by the \textbf{Ours} model show the greatest combination of emotion and variation, making for the most human-like model.}
\end{table*}


\begin{table*}[]
\begin{tabular}{l|l}
\hline
Ours-No-Emote & Ours \\
  \hline
  \hline
  \multicolumn{3}{c}{Finding: recurrent headache  Emote: affirmative } \\
  \multicolumn{3}{c}{Expert: Do you have headaches that come and go often?} \\
  \hline
  Do you have headaches that occur on a regular basis?  & Thanks for the input. Does you  headache keep coming back?\\
 Are your headaches recurring? & Okay. Is your headache recurrent?  \\
\end{tabular}
\label{tab:qual_comparison}
\caption{Qualitative comparison of generated questions by the three NLG models. Note the lack of diversity in the \textbf{Expert} model and lack of emotion in the \textbf{Ours-no-Emote} model. The questions generated by the \textbf{Ours} model show the greatest combination of emotion and variation, making for the most human-like model.}
\end{table*}



==> sections/simulation.tex <==
\begin{algorithm}[t]
    \caption{Active Long-Tailed Learning (ALTL)} \label{alg}
    \begin{algorithmic}[1]
        \renewcommand{\algorithmicrequire}{\textbf{Input:}}
        \renewcommand{\algorithmicensure}{\textbf{Output:}}
        \REQUIRE Labeled set $D_L$, Unlabeled pool $D_U$, Budget $b$, Feature extractor $f(.)$
        \STATE Initialize $n = |D_L|$
        \STATE $r_1, \dots, r_p \gets \textsc{Affinity}(f(D_L \cup D_U))$
        \REPEAT 
        \STATE $u \gets \textsc{GetDatumToLabel}$($D_L$,$D_U$, $r_1, \dots, r_p, f(.)$)
        %\vspace{-10pt}
        \STATE $y = \textsc{Oracle}(u)$
        \STATE$ D_L = D_L \cup \{(u, y)\}$
        \STATE$ D_U = D_U - \{u\}$
        \UNTIL $|D_L| = n + b$
        \RETURN $D_L$ and $D_U$
    \end{algorithmic} 
\end{algorithm}


